Cosmology from HI galaxy surveys with the SKA

The Square Kilometer Array (SKA) has the potential to produce galaxy redshift surveys which will be competitive with other state of the art cosmological experiments in the next decade. In this chapter we summarise what capabilities the first and the second phases of the SKA will be able to achieve in its current state of design. We summarise the different cosmological experiments which are outlined in further detail in other chapters of this Science Book. The SKA will be able to produce competitive Baryonic Oscillation (BAOs) measurements in both its phases. The first phase of the SKA will provide similar measurements as optical and IR experiments with completely different systematic effects whereas the second phase being transformational in terms of its statistical power. The SKA will produce very accurate Redshift Space Distortions (RSD) measurements, being superior to other experiments at lower redshifts, due to the large number of galaxies. Cross correlations of the galaxy redshift data from the SKA with radio continuum surveys and optical surveys will provide extremely good calibration of photometric redshifts as well as extremely good bounds on modifications of gravity. Basing on a Principle Component Analysis (PCA) approach, we find that the SKA will be able to provide competitive constraints on dark energy and modified gravity models. Due to the large area covered the SKA it will be a transformational experiment in measuring physics from the largest scales such as non-Gaussian signals from $\textrm{f}_{\textrm{nl}}$. Finally, the SKA might produce the first real time measurement of the redshift drift. The SKA will be a transformational machine for cosmology as it grows from an early Phase 1 to its full power.

==> aa.tex <==
@ARTICLE{2011ApJ...727...40F,
   author = {{Freudling}, W. and {Staveley-Smith}, L. and {Catinella}, B. and 
	{Minchin}, R. and {Calabretta}, M. and {Momjian}, E. and {Zwaan}, M. and 
	{Meyer}, M. and {O'Neil}, K.},
    title = "{Deep 21 cm H I Observations at z {$\sim$} 0.1: The Precursor to the Arecibo Ultra Deep Survey}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1011.0877},
 primaryClass = "astro-ph.CO",
 keywords = {cosmology: observations, galaxies: evolution, radio lines: galaxies},
     year = 2011,
    month = jan,
   volume = 727,
      eid = {40},
    pages = {40},
      doi = {10.1088/0004-637X/727/1/40},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...727...40F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013arXiv1303.5077P,
   author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and 
	{Armitage-Caplan}, C. and {Arnaud}, M. and {Ashdown}, M. and 
	{Atrio-Barandela}, F. and {Aumont}, J. and {Baccigalupi}, C. and 
	{Banday}, A.~J. and et al.},
    title = "{Planck 2013 results. XVII. Gravitational lensing by large-scale structure}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1303.5077},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2013,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1303.5077P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{IMSANTOS,
   author = {{Santos}, M. G. and others},
    title = "{Intensity Mappting with the SKA}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}

@INPROCEEDINGS{CONTJARVIS,
   author = {{Jarvis}, M. J. and others},
    title = "{Continuum surveys with the SKA}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}

@INPROCEEDINGS{HANSPROC,
   author = {{Kl\"ockner}, H.-R.},
    title = "{astro-ph\textbackslash 1301.4124}",
    booktitle = {Pathway to the SKA - The German White Paper, eds. H.-R. Kl\"ockner,M. Kramer, H. Falcke, D. Schwarz, A. Eckart, G. Kauffmann},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}

@INPROCEEDINGS{santosSKAdndz,
   author = {{Santos}, M. G. and others},
    title = "{HI galaxy simulations: number counts and bias}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}


@INPROCEEDINGS{Camera:SKACHAP,
   author = {{Camera}, S. and others},
    title = "{Cosmology at large scales with the SKA}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}

@INPROCEEDINGS{SKABAO,
   author = {{Bull}, P. and others},
    title = "{SKA BAO Chapter}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}

@ARTICLE{2013arXiv1303.5076P,
   author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and 
	{Armitage-Caplan}, C. and {Arnaud}, M. and {Ashdown}, M. and 
	{Atrio-Barandela}, F. and {Aumont}, J. and {Baccigalupi}, C. and 
	{Banday}, A.~J. and et al.},
    title = "{Planck 2013 results. XVI. Cosmological parameters}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1303.5076},
 primaryClass = "astro-ph.CO",
 keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
     year = 2013,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1303.5076P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{SKACROSS,
   author = {{Kirk}, D. and others},
    title = "{Cross correlation surveys with the SKA}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}

@INPROCEEDINGS{SKARSD,
   author = {{Raccanelli}, A.  and others},
    title = "{SKA RSD Chapter}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}

@INPROCEEDINGS{SKAPCA,
   author = {{Zhao}, G.~B.  and others},
    title = "{SKA PCA Chapter}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}


@ARTICLE{2009ApJ...703.1890O,
   author = {{Obreschkow}, D. and {Kl{\"o}ckner}, H.-R. and {Heywood}, I. and 
	{Levrier}, F. and {Rawlings}, S.},
    title = "{A Virtual Sky with Extragalactic H I and CO Lines for the Square Kilometre Array and the Atacama Large Millimeter/Submillimeter Array}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0908.0983},
 primaryClass = "astro-ph.CO",
 keywords = {cosmology: theory, galaxies: evolution, galaxies: high-redshift, ISM: atoms, ISM: molecules},
     year = 2009,
    month = oct,
   volume = 703,
    pages = {1890-1903},
      doi = {10.1088/0004-637X/703/2/1890},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...703.1890O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013arXiv1303.5084P,
   author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and 
	{Armitage-Caplan}, C. and {Arnaud}, M. and {Ashdown}, M. and 
	{Atrio-Barandela}, F. and {Aumont}, J. and {Baccigalupi}, C. and 
	{Banday}, A.~J. and et al.},
    title = "{Planck 2013 Results. XXIV. Constraints on primordial non-Gaussianity}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1303.5084},
 primaryClass = "astro-ph.CO",
 keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
     year = 2013,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1303.5084P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2012MNRAS.427.3435A,
   author = {{Anderson}, L. and et al.},
    title = "{The clustering of galaxies in the SDSS-III Baryon Oscillation Spectroscopic Survey: baryon acoustic oscillations in the Data Release 9 spectroscopic galaxy sample}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1203.6594},
 primaryClass = "astro-ph.CO",
 keywords = {cosmological parameters, cosmology: observations, dark energy, distance scale, large-scale structure of Universe},
     year = 2012,
    month = dec,
   volume = 427,
    pages = {3435-3467},
      doi = {10.1111/j.1365-2966.2012.22066.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.427.3435A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.422.2854G,
   author = {{Giannantonio}, T. and {Porciani}, C. and {Carron}, J. and {Amara}, A. and 
	{Pillepich}, A.},
    title = "{Constraining primordial non-Gaussianity with future galaxy surveys}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1109.0958},
 primaryClass = "astro-ph.CO",
 keywords = {cosmological parameters, early Universe, large-scale structure of the Universe},
     year = 2012,
    month = jun,
   volume = 422,
    pages = {2854-2877},
      doi = {10.1111/j.1365-2966.2012.20604.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.422.2854G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014PhRvD..89b3511G,
   author = {{Giannantonio}, T. and {Ross}, A.~J. and {Percival}, W.~J. and 
	{Crittenden}, R. and {Bacher}, D. and {Kilbinger}, M. and {Nichol}, R. and 
	{Weller}, J.},
    title = "{Improved primordial non-Gaussianity constraints from measurements of galaxy clustering and the integrated Sachs-Wolfe effect}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1303.1349},
 primaryClass = "astro-ph.CO",
 keywords = {Observational cosmology, Superclusters, large-scale structure of the Universe},
     year = 2014,
    month = jan,
   volume = 89,
   number = 2,
      eid = {023511},
    pages = {023511},
      doi = {10.1103/PhysRevD.89.023511},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..89b3511G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008PhRvD..77l3514D,
   author = {{Dalal}, N. and {Dor{\'e}}, O. and {Huterer}, D. and {Shirokov}, A.
	},
    title = "{Imprints of primordial non-Gaussianities on large-scale structure: Scale-dependent bias and abundance of virialized objects}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {0710.4560},
 keywords = {Superclusters, large-scale structure of the Universe, Dark matter, Particle-theory and field-theory models of the early Universe},
     year = 2008,
    month = jun,
   volume = 77,
   number = 12,
      eid = {123514},
    pages = {123514},
      doi = {10.1103/PhysRevD.77.123514},
   adsurl = {http://adsabs.harvard.edu/abs/2008PhRvD..77l3514D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008ApJ...677L..77M,
   author = {{Matarrese}, S. and {Verde}, L.},
    title = "{The Effect of Primordial Non-Gaussianity on Halo Bias}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0801.4826},
 keywords = {Cosmology: Theory, Galaxies: Clusters: General, Galaxies: Halos, Cosmology: Large-Scale Structure of Universe},
     year = 2008,
    month = apr,
   volume = 677,
    pages = {L77-L80},
      doi = {10.1086/587840},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...677L..77M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013PhRvL.111q1302C,
   author = {{Camera}, S. and {Santos}, M.~G. and {Ferreira}, P.~G. and {Ferramacho}, L.
	},
    title = "{Cosmology on Ultralarge Scales with Intensity Mapping of the Neutral Hydrogen 21 cm Emission: Limits on Primordial Non-Gaussianity}",
  journal = {Physical Review Letters},
archivePrefix = "arXiv",
   eprint = {1305.6928},
 primaryClass = "astro-ph.CO",
 keywords = {Cosmology, HI regions and 21-cm lines, diffuse translucent and high-velocity clouds, Radio sources},
     year = 2013,
    month = oct,
   volume = 111,
   number = 17,
      eid = {171302},
    pages = {171302},
      doi = {10.1103/PhysRevLett.111.171302},
   adsurl = {http://adsabs.harvard.edu/abs/2013PhRvL.111q1302C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009PhRvL.102b1302S,
   author = {{Seljak}, U.},
    title = "{Extracting Primordial Non-Gaussianity without Cosmic Variance}",
  journal = {Physical Review Letters},
archivePrefix = "arXiv",
   eprint = {0807.1770},
 keywords = {Observational cosmology, Superclusters, large-scale structure of the Universe},
     year = 2009,
    month = jan,
   volume = 102,
   number = 2,
      eid = {021302},
    pages = {021302},
      doi = {10.1103/PhysRevLett.102.021302},
   adsurl = {http://adsabs.harvard.edu/abs/2009PhRvL.102b1302S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002ApJ...565....1G,
   author = {{Gudmundsson}, E.~H. and {Bj{\"o}rnsson}, G.},
    title = "{Dark Energy and the Observable Universe}",
  journal = {\apj},
   eprint = {astro-ph/0105547},
 keywords = {Cosmology: Observations, Cosmology: Theory, Relativity},
     year = 2002,
    month = jan,
   volume = 565,
    pages = {1-16},
      doi = {10.1086/324496},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...565....1G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1962ApJ...136..319S,
   author = {{Sandage}, A.},
    title = "{The Change of Redshift and Apparent Luminosity of Galaxies due to the Deceleration of Selected Expanding Universes.}",
  journal = {\apj},
     year = 1962,
    month = sep,
   volume = 136,
    pages = {319},
      doi = {10.1086/147385},
   adsurl = {http://adsabs.harvard.edu/abs/1962ApJ...136..319S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005Msngr.122...10P,
   author = {{Pasquini}, L. and {Cristiani}, S. and {Dekker}, H. and {Haehnelt}, M. and 
	{Molaro}, P. and {Pepe}, F. and {Avila}, G. and {Delabre}, B. and 
	{D'Odorico}, S. and {Liske}, J. and {Shaver}, P. and {Bonifacio}, P. and 
	{Borgani}, S. and {D'Odorico}, V. and {Vanzella}, E. and {Bouchy}, F. and 
	{Dessauges-Lavadsky}, M. and {Lovis}, C. and {Mayor}, M. and 
	{Queloz}, D. and {Udry}, S. and {Murphy}, M. and {Viel}, M. and 
	{Grazian}, A. and {Levshakov}, S. and {Moscardini}, L. and {Wiklind}, T. and 
	{Zucker}, S.},
    title = "{CODEX: Measuring the Expansion of the Universe (and beyond)}",
  journal = {The Messenger},
     year = 2005,
    month = dec,
   volume = 122,
    pages = {10-14},
   adsurl = {http://adsabs.harvard.edu/abs/2005Msngr.122...10P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Camera:2014bwa,
      author         = {{Camera}, ~S. and {Santos}, ~M.~G. and {Maartens}, R.},
      title          = "{Probing primordial non-Gaussianity with SKA galaxy
                        redshift surveys: a fully relativistic analysis}",
      journal = {},
      year           = "2014",
      eprint         = "1409.8286",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1409.8286;%%",
}


@ARTICLE{2014MNRAS.442.2511F,
   author = {{Ferramacho}, L.~D. and {Santos}, M.~G. and {Jarvis}, M.~J. and 
	{Camera}, S.},
    title = "{Radio galaxy populations and the multitracer technique: pushing the limits on primordial non-Gaussianity}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1402.2290},
 primaryClass = "astro-ph.CO",
 keywords = {cosmological parameters, cosmology: observations, inflation, large-scale structure of Universe, radio continuum: galaxies},
     year = 2014,
    month = aug,
   volume = 442,
    pages = {2511-2518},
      doi = {10.1093/mnras/stu1015},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.442.2511F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJS..208...19H,
   author = {{Hinshaw}, G. and {Larson}, D. and {Komatsu}, E. and {Spergel}, D.~N. and 
	{Bennett}, C.~L. and {Dunkley}, J. and {Nolta}, M.~R. and {Halpern}, M. and 
	{Hill}, R.~S. and {Odegard}, N. and {Page}, L. and {Smith}, K.~M. and 
	{Weiland}, J.~L. and {Gold}, B. and {Jarosik}, N. and {Kogut}, A. and 
	{Limon}, M. and {Meyer}, S.~S. and {Tucker}, G.~S. and {Wollack}, E. and 
	{Wright}, E.~L.},
    title = "{Nine-year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Parameter Results}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1212.5226},
 primaryClass = "astro-ph.CO",
 keywords = {cosmic background radiation, cosmology: observations, dark matter, early universe, instrumentation: detectors, space vehicles, space vehicles: instruments, telescopes },
     year = 2013,
    month = oct,
   volume = 208,
      eid = {19},
    pages = {19},
      doi = {10.1088/0067-0049/208/2/19},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJS..208...19H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{1998ApJ...499L.111L,
   author = {{Loeb}, A.},
    title = "{Direct Measurement of Cosmological Parameters from the Cosmic Deceleration of Extragalactic Objects}",
  journal = {\apjl},
   eprint = {astro-ph/9802122},
 keywords = {COSMOLOGY: THEORY, Cosmology: Theory},
     year = 1998,
    month = jun,
   volume = 499,
    pages = {L111-L114},
      doi = {10.1086/311375},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...499L.111L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> cosmology-galaxy-surveys 2/aa.tex <==
@ARTICLE{2011ApJ...727...40F,
   author = {{Freudling}, W. and {Staveley-Smith}, L. and {Catinella}, B. and 
	{Minchin}, R. and {Calabretta}, M. and {Momjian}, E. and {Zwaan}, M. and 
	{Meyer}, M. and {O'Neil}, K.},
    title = "{Deep 21 cm H I Observations at z {$\sim$} 0.1: The Precursor to the Arecibo Ultra Deep Survey}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1011.0877},
 primaryClass = "astro-ph.CO",
 keywords = {cosmology: observations, galaxies: evolution, radio lines: galaxies},
     year = 2011,
    month = jan,
   volume = 727,
      eid = {40},
    pages = {40},
      doi = {10.1088/0004-637X/727/1/40},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...727...40F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013arXiv1303.5077P,
   author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and 
	{Armitage-Caplan}, C. and {Arnaud}, M. and {Ashdown}, M. and 
	{Atrio-Barandela}, F. and {Aumont}, J. and {Baccigalupi}, C. and 
	{Banday}, A.~J. and et al.},
    title = "{Planck 2013 results. XVII. Gravitational lensing by large-scale structure}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1303.5077},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2013,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1303.5077P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{IMSANTOS,
   author = {{Santos}, M. G. and others},
    title = "{Intensity Mappting with the SKA}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}

@INPROCEEDINGS{CONTJARVIS,
   author = {{Jarvis}, M. J. and others},
    title = "{Continuum surveys with the SKA}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}

@INPROCEEDINGS{HANSPROC,
   author = {{Kl\"ockner}, H.-R.},
    title = "{astro-ph\textbackslash 1301.4124}",
    booktitle = {Pathway to the SKA - The German White Paper, eds. H.-R. Kl\"ockner,M. Kramer, H. Falcke, D. Schwarz, A. Eckart, G. Kauffmann},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}

@INPROCEEDINGS{santosSKAdndz,
   author = {{Santos}, M. G. and others},
    title = "{HI galaxy simulations: number counts and bias}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}


@INPROCEEDINGS{Camera:SKACHAP,
   author = {{Camera}, S. and others},
    title = "{Cosmology at large scales with the SKA}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}

@INPROCEEDINGS{SKABAO,
   author = {{Bull}, P. and others},
    title = "{SKA BAO Chapter}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}

@ARTICLE{2013arXiv1303.5076P,
   author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and 
	{Armitage-Caplan}, C. and {Arnaud}, M. and {Ashdown}, M. and 
	{Atrio-Barandela}, F. and {Aumont}, J. and {Baccigalupi}, C. and 
	{Banday}, A.~J. and et al.},
    title = "{Planck 2013 results. XVI. Cosmological parameters}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1303.5076},
 primaryClass = "astro-ph.CO",
 keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
     year = 2013,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1303.5076P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{SKACROSS,
   author = {{Kirk}, D. and others},
    title = "{Cross correlation surveys with the SKA}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}

@INPROCEEDINGS{SKARSD,
   author = {{Raccanelli}, A.  and others},
    title = "{SKA RSD Chapter}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}

@INPROCEEDINGS{SKAPCA,
   author = {{Zhao}, G.~B.  and others},
    title = "{SKA PCA Chapter}",
    booktitle = {Advancing Astrophysics with the Square Kilometre Array},
     year = 2014,
    month = dec,
    pages = {},
    series = {PoS(AASKA14)},
   editor = {},
   adsurl = {},
  adsnote = {}
}


@ARTICLE{2009ApJ...703.1890O,
   author = {{Obreschkow}, D. and {Kl{\"o}ckner}, H.-R. and {Heywood}, I. and 
	{Levrier}, F. and {Rawlings}, S.},
    title = "{A Virtual Sky with Extragalactic H I and CO Lines for the Square Kilometre Array and the Atacama Large Millimeter/Submillimeter Array}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0908.0983},
 primaryClass = "astro-ph.CO",
 keywords = {cosmology: theory, galaxies: evolution, galaxies: high-redshift, ISM: atoms, ISM: molecules},
     year = 2009,
    month = oct,
   volume = 703,
    pages = {1890-1903},
      doi = {10.1088/0004-637X/703/2/1890},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...703.1890O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013arXiv1303.5084P,
   author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and 
	{Armitage-Caplan}, C. and {Arnaud}, M. and {Ashdown}, M. and 
	{Atrio-Barandela}, F. and {Aumont}, J. and {Baccigalupi}, C. and 
	{Banday}, A.~J. and et al.},
    title = "{Planck 2013 Results. XXIV. Constraints on primordial non-Gaussianity}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1303.5084},
 primaryClass = "astro-ph.CO",
 keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
     year = 2013,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1303.5084P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2012MNRAS.427.3435A,
   author = {{Anderson}, L. and et al.},
    title = "{The clustering of galaxies in the SDSS-III Baryon Oscillation Spectroscopic Survey: baryon acoustic oscillations in the Data Release 9 spectroscopic galaxy sample}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1203.6594},
 primaryClass = "astro-ph.CO",
 keywords = {cosmological parameters, cosmology: observations, dark energy, distance scale, large-scale structure of Universe},
     year = 2012,
    month = dec,
   volume = 427,
    pages = {3435-3467},
      doi = {10.1111/j.1365-2966.2012.22066.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.427.3435A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.422.2854G,
   author = {{Giannantonio}, T. and {Porciani}, C. and {Carron}, J. and {Amara}, A. and 
	{Pillepich}, A.},
    title = "{Constraining primordial non-Gaussianity with future galaxy surveys}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1109.0958},
 primaryClass = "astro-ph.CO",
 keywords = {cosmological parameters, early Universe, large-scale structure of the Universe},
     year = 2012,
    month = jun,
   volume = 422,
    pages = {2854-2877},
      doi = {10.1111/j.1365-2966.2012.20604.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.422.2854G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014PhRvD..89b3511G,
   author = {{Giannantonio}, T. and {Ross}, A.~J. and {Percival}, W.~J. and 
	{Crittenden}, R. and {Bacher}, D. and {Kilbinger}, M. and {Nichol}, R. and 
	{Weller}, J.},
    title = "{Improved primordial non-Gaussianity constraints from measurements of galaxy clustering and the integrated Sachs-Wolfe effect}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1303.1349},
 primaryClass = "astro-ph.CO",
 keywords = {Observational cosmology, Superclusters, large-scale structure of the Universe},
     year = 2014,
    month = jan,
   volume = 89,
   number = 2,
      eid = {023511},
    pages = {023511},
      doi = {10.1103/PhysRevD.89.023511},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..89b3511G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008PhRvD..77l3514D,
   author = {{Dalal}, N. and {Dor{\'e}}, O. and {Huterer}, D. and {Shirokov}, A.
	},
    title = "{Imprints of primordial non-Gaussianities on large-scale structure: Scale-dependent bias and abundance of virialized objects}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {0710.4560},
 keywords = {Superclusters, large-scale structure of the Universe, Dark matter, Particle-theory and field-theory models of the early Universe},
     year = 2008,
    month = jun,
   volume = 77,
   number = 12,
      eid = {123514},
    pages = {123514},
      doi = {10.1103/PhysRevD.77.123514},
   adsurl = {http://adsabs.harvard.edu/abs/2008PhRvD..77l3514D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008ApJ...677L..77M,
   author = {{Matarrese}, S. and {Verde}, L.},
    title = "{The Effect of Primordial Non-Gaussianity on Halo Bias}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0801.4826},
 keywords = {Cosmology: Theory, Galaxies: Clusters: General, Galaxies: Halos, Cosmology: Large-Scale Structure of Universe},
     year = 2008,
    month = apr,
   volume = 677,
    pages = {L77-L80},
      doi = {10.1086/587840},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...677L..77M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013PhRvL.111q1302C,
   author = {{Camera}, S. and {Santos}, M.~G. and {Ferreira}, P.~G. and {Ferramacho}, L.
	},
    title = "{Cosmology on Ultralarge Scales with Intensity Mapping of the Neutral Hydrogen 21 cm Emission: Limits on Primordial Non-Gaussianity}",
  journal = {Physical Review Letters},
archivePrefix = "arXiv",
   eprint = {1305.6928},
 primaryClass = "astro-ph.CO",
 keywords = {Cosmology, HI regions and 21-cm lines, diffuse translucent and high-velocity clouds, Radio sources},
     year = 2013,
    month = oct,
   volume = 111,
   number = 17,
      eid = {171302},
    pages = {171302},
      doi = {10.1103/PhysRevLett.111.171302},
   adsurl = {http://adsabs.harvard.edu/abs/2013PhRvL.111q1302C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009PhRvL.102b1302S,
   author = {{Seljak}, U.},
    title = "{Extracting Primordial Non-Gaussianity without Cosmic Variance}",
  journal = {Physical Review Letters},
archivePrefix = "arXiv",
   eprint = {0807.1770},
 keywords = {Observational cosmology, Superclusters, large-scale structure of the Universe},
     year = 2009,
    month = jan,
   volume = 102,
   number = 2,
      eid = {021302},
    pages = {021302},
      doi = {10.1103/PhysRevLett.102.021302},
   adsurl = {http://adsabs.harvard.edu/abs/2009PhRvL.102b1302S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002ApJ...565....1G,
   author = {{Gudmundsson}, E.~H. and {Bj{\"o}rnsson}, G.},
    title = "{Dark Energy and the Observable Universe}",
  journal = {\apj},
   eprint = {astro-ph/0105547},
 keywords = {Cosmology: Observations, Cosmology: Theory, Relativity},
     year = 2002,
    month = jan,
   volume = 565,
    pages = {1-16},
      doi = {10.1086/324496},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...565....1G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1962ApJ...136..319S,
   author = {{Sandage}, A.},
    title = "{The Change of Redshift and Apparent Luminosity of Galaxies due to the Deceleration of Selected Expanding Universes.}",
  journal = {\apj},
     year = 1962,
    month = sep,
   volume = 136,
    pages = {319},
      doi = {10.1086/147385},
   adsurl = {http://adsabs.harvard.edu/abs/1962ApJ...136..319S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005Msngr.122...10P,
   author = {{Pasquini}, L. and {Cristiani}, S. and {Dekker}, H. and {Haehnelt}, M. and 
	{Molaro}, P. and {Pepe}, F. and {Avila}, G. and {Delabre}, B. and 
	{D'Odorico}, S. and {Liske}, J. and {Shaver}, P. and {Bonifacio}, P. and 
	{Borgani}, S. and {D'Odorico}, V. and {Vanzella}, E. and {Bouchy}, F. and 
	{Dessauges-Lavadsky}, M. and {Lovis}, C. and {Mayor}, M. and 
	{Queloz}, D. and {Udry}, S. and {Murphy}, M. and {Viel}, M. and 
	{Grazian}, A. and {Levshakov}, S. and {Moscardini}, L. and {Wiklind}, T. and 
	{Zucker}, S.},
    title = "{CODEX: Measuring the Expansion of the Universe (and beyond)}",
  journal = {The Messenger},
     year = 2005,
    month = dec,
   volume = 122,
    pages = {10-14},
   adsurl = {http://adsabs.harvard.edu/abs/2005Msngr.122...10P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Camera:2014bwa,
      author         = {{Camera}, ~S. and {Santos}, ~M.~G. and {Maartens}, R.},
      title          = "{Probing primordial non-Gaussianity with SKA galaxy
                        redshift surveys: a fully relativistic analysis}",
      journal = {},
      year           = "2014",
      eprint         = "1409.8286",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1409.8286;%%",
}


@ARTICLE{2014MNRAS.442.2511F,
   author = {{Ferramacho}, L.~D. and {Santos}, M.~G. and {Jarvis}, M.~J. and 
	{Camera}, S.},
    title = "{Radio galaxy populations and the multitracer technique: pushing the limits on primordial non-Gaussianity}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1402.2290},
 primaryClass = "astro-ph.CO",
 keywords = {cosmological parameters, cosmology: observations, inflation, large-scale structure of Universe, radio continuum: galaxies},
     year = 2014,
    month = aug,
   volume = 442,
    pages = {2511-2518},
      doi = {10.1093/mnras/stu1015},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.442.2511F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJS..208...19H,
   author = {{Hinshaw}, G. and {Larson}, D. and {Komatsu}, E. and {Spergel}, D.~N. and 
	{Bennett}, C.~L. and {Dunkley}, J. and {Nolta}, M.~R. and {Halpern}, M. and 
	{Hill}, R.~S. and {Odegard}, N. and {Page}, L. and {Smith}, K.~M. and 
	{Weiland}, J.~L. and {Gold}, B. and {Jarosik}, N. and {Kogut}, A. and 
	{Limon}, M. and {Meyer}, S.~S. and {Tucker}, G.~S. and {Wollack}, E. and 
	{Wright}, E.~L.},
    title = "{Nine-year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Parameter Results}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1212.5226},
 primaryClass = "astro-ph.CO",
 keywords = {cosmic background radiation, cosmology: observations, dark matter, early universe, instrumentation: detectors, space vehicles, space vehicles: instruments, telescopes },
     year = 2013,
    month = oct,
   volume = 208,
      eid = {19},
    pages = {19},
      doi = {10.1088/0067-0049/208/2/19},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJS..208...19H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{1998ApJ...499L.111L,
   author = {{Loeb}, A.},
    title = "{Direct Measurement of Cosmological Parameters from the Cosmic Deceleration of Extragalactic Objects}",
  journal = {\apjl},
   eprint = {astro-ph/9802122},
 keywords = {COSMOLOGY: THEORY, Cosmology: Theory},
     year = 1998,
    month = jun,
   volume = 499,
    pages = {L111-L114},
      doi = {10.1086/311375},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...499L.111L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

